On Multi-objective Policy Optimization as a Tool for Reinforcement Learning: Case Studies in Offline RL and Finetuning

Many advances that have improved the robustness and efficiency of deep reinforcement learning (RL) algorithms can, in one way or another, be understood as introducing additional objectives or constraints in the policy optimization step. This includes ideas as far ranging as exploration bonuses, entropy regularization, and regularization toward teachers or data priors. Often, the task reward and auxiliary objectives are in conflict, and in this paper we argue that this makes it natural to treat these cases as instances of multi-objective (MO) optimization problems. We demonstrate how this perspective allows us to develop novel and more effective RL algorithms. In particular, we focus on offline RL and finetuning as case studies, and show that existing approaches can be understood as MO algorithms relying on linear scalarization. We hypothesize that replacing linear scalarization with a better algorithm can improve performance. We introduce Distillation of a Mixture of Experts (DiME), a new MORL algorithm that outperforms linear scalarization and can be applied to these non-standard MO problems. We demonstrate that for offline RL, DiME leads to a simple new algorithm that outperforms state-of-the-art. For finetuning, we derive new algorithms that learn to outperform the teacher policy.

==> 04_approach_old.tex <==
\section{Distillation of a Mixture of Experts (DiME) \textcolor{purple}{[Second Version]}}

Consider the projection view on policy improvement in RL, which consists of two steps: first, find an improved policy with respect to an objective (\emph{e.g.,} the critic in actor-critic methods, or a Monte Carlo return estimate in REINFORCE); and second, project this improved policy back into the space of allowed policies, usually a parametric space that facilitates sampling.
%we are interested in via supervised learning.

In this section we show that depending on our design choice, we can enforce our desired preference
trade-off either in the improvement step or the projection step. In what follows we consider the KL 
regularised policy objective, computed at a given state $s$ as
\begin{align}
    J(q; s) = \mathbb{E}_{a \sim q(\cdot|s)}Q(a, s) - \eta \mathrm{KL}\left( q(\cdot|s) | \pi_{\theta_t}(\cdot|s) \right),
\label{equ:single-objective-policy-objective}
\end{align}
where $\eta$ is a Lagrange dual variable maintaining a safe distance from the previous iterate $\pi_t$.

\paragraph{Improvement}
In this step, the policy objective $J$ is maximized by the following known nonparametric solution~\aanote{add citations}:
\begin{equation}
    q(a|s) \propto \pi_{\theta_t}(a|s) \exp\left(\frac{Q(a,s)}{\eta}\right),
\end{equation}
producing an improved policy $q$, which does not necessarily lie in the allowed family of policies (perhaps it is not amenable to efficient 
sampling).

\paragraph{Projection}
Next we project the improved policies $q$ into the space of policies we are interested in via the following minimization:
\begin{equation}
    \theta_{t+1} = \argmin_{\theta} \mathbb{E}_{\mu(s)}\Big[\mathrm{KL}\Big(q(\cdot | s) \, \| \, \pi_{\theta}(\cdot | s)\Big)\Big].
\label{eq:klmin}
\end{equation}

\subsection{Multi-objective extensions}
In this work we consider a natural extension to the notion of improvement, measured via a 
convex combination of $K$ objectives denoted $\{Q_k\}_k$,
where the associated preference trade-off coefficients $\{\alpha_k\}_k$ sum to 1.
Note that while we denote the multiple objective functions as $Q_k$, this formulation trivially extends
to objective functions that are not related to a state-action value estimate of an environment return,
as indeed we present in several case studies below.

% \paragraph{Improvement}
% In order to calculate the improved policies we generalise the KL regularised RL objective for multi-objective optimisation, i.e,
Consider a simple multi-objective extension of \eqref{equ:single-objective-policy-objective}
where we allow for a KL regularized improved policy $q_k$ per objective $Q_k$, so that the 
multi-objective policy objective becomes
\begin{equation}
    J_K(\{q_k\}_k; s)
    = \sum_{k=1}^K \alpha_k \left[
        \mathbb{E}_{a \sim q_{k}(\cdot|s)} Q_k(a,s)
        - \eta_k \mathrm{KL}\left(q_k(\cdot|s) | \pi_t(\cdot|s)\right)
    \right],
\end{equation}
which can be maximized independently for each objective, each with the following known nonparametric 
solution~\aanote{add citations}.
\begin{equation}
    q_k(a|s) \propto \pi_t(a|s) \exp\left(\frac{Q_k(a,s)}{\eta_k}\right).
\end{equation}
We can see in this case that the preference coefficients $\alpha_k$ have no effect in obtaining the 
per-objective improved policies $q_k$ and indeed the preference trade-off only impact the projection step by the following
weighted projection of the improved policies into a single $\pi_{\theta_{t+1}}$ via the following supervised learning iteration:
\begin{equation}
    \theta_{t+1}
    = \argmin_{\theta} \sum_{k=1}^N \alpha_k \mathbb{E}_{\mu(s)}\Big[\mathrm{KL}\Big(q_k(a | s) \, \| \, \pi_{\theta}(a | s)\Big)\Big].
\label{eq:klmin-multi}
\end{equation}
One of the benefits of this specification of preferences is that it is done in a scale-invariant way; notice that the coefficients
$\alpha_k$ never multiply the objective functions $Q_k$, which can be in arbitrary scales.
 
\subsection{Linear scalarization: specifying preferences in the improvement step} 

Alternatively, consider the result of the improvement step had we chosen to identify a single improved
policy $q$ for all the objectives as follows:
\begin{equation}
    J_S(q; s) = J_K(\{q\}_k; s)
    = \mathbb{E}_{a \sim q(\cdot|s)} \sum_{k=1}^K \alpha_k Q_{k}(a,s)
    - \left(\sum_{k=1}^K \alpha_k\eta_k\right) \mathrm{KL}\left(q(\cdot|s) | \pi_t(\cdot|s)\right),
\end{equation}
which yields the typical linear scalarized objective solution:
\begin{equation}
    q(a|s) \propto \pi_t(a|s) \exp\left(\frac{\sum_{k=1}^K \alpha_k Q_{k}(a,s)}{\eta}\right),
\end{equation}
where $\eta = \sum_{k=1}^K \alpha_k\eta_k$. Finally, as there is a single policy to project, the projection step is identical
to~\eqref{eq:klmin} and the preferences over objectives does not have any further effect.


\subsection{DiME: specifying preferences in the projection step} 

\subsection{Theoretical Analysis}
DiME is able to find solutions on the Pareto front that linear scalarization cannot. {\textcolor{purple} {[add theoretical proofs here]}}

\subsection{Offline RL}
In this section we consider learning a task from experts.
In addition to a task reward produced by the environment, we have access to expert information, either in the form of sampled experiential data (in the case of offline RL) or a stochastic policy we can query (in the case of kickstarting).
% experts can have different forms including a parametric form (such as pre-trained policies) and state-action transitions or both.
Our goal is to exploit the expert data and the task reward such that we learn a given task more efficiently.
We model this problem as a multi-objective problem with two objectives:
\begin{enumerate}
\item optimizing for the task return, and
\item staying close to the expert data.
\end{enumerate}

This is a general framework that allows for several design choices.
In particular, we need to formalize the mathematical objective functions corresponding to each objective.
We model learning a task given an expert policy $\pi_e(a|s)$ as a multi-objective problem with the following objective functions:
% For that we define two following Q-functions to evaluate actions from the policy $\pi_{old}(a|s)$ in state $s$:
\begin{enumerate}
\item the task Q-function $Q(a,s)$ learned via bootstrapping and
\item the log-probability ratio $\log\frac{\pi_{e}(a|s)}{\pi_t(a|s)}$.
\end{enumerate}
In what follows we compare linear scalarization and our proposed multi-objective approach by deriving their corresponding policy losses.

\subsubsection{Multi-objective RL via Linear Scalarization}
\label{sec:method_linear}
A simple baseline approach to optimize both objectives is to use a weighted linear combination of the two objective functions with a preference
trade-off $\alpha \in [0, 1]$ to specify the importance of each.
Evaluated at an arbitrary state $s$, this leads to the following single objective function to maximize:
\begin{align}
    \mathbb{E}_{a \sim \pi_\theta} \left[
        (1 - \alpha) \frac{Q(a,s)}{\lambda} + \alpha \log \frac{\pi_{e}(a|s)}{\pi_t(a|s)}
    \right],
\end{align}
where $\lambda > 0$ is used to scale the $Q$-values appropriately so that the trade-off parameter $\alpha$ takes reasonable values.
Let us now use MPO to optimize this objective in a constrained way, staying close to the previous iterate $\pi_t$, leading to the following objective to maximize:
\begin{align}
    J_S(\theta; s)
    &= \int\pi_t(a|s)
    \exp\left[
        (1 - \alpha) \frac{Q(a,s)}{\lambda\eta} + \frac{\alpha}{\eta} \log \frac{\pi_{e}(a|s)}{\pi_t(a|s)}
    \right] \log \pi_{\theta}(a|s),
\intertext{where setting the dual variable $\eta=\alpha$ yields}
    &= \int\pi_t(a|s)\frac{\pi_{e}(a|s)}{\pi_t(a|s)}\exp\left[ \frac{(1 - \alpha) Q(a,s)}{\alpha \lambda}\right] \log \pi_{\theta}(a|s)
\intertext{after cancelling out and rearranging terms:}
    &= \int\pi_{e}(a|s)\exp\left[\frac{Q(a,s)}{\beta}\right] \log \pi_{\theta}(a|s)
    \label{eq:awbc}
\end{align}
where we've adopted $\beta$ as the temperature hyperparameter used in offline RL algorithms such as CRR~\citep{Wang_2020}, revealing the similarities between this scalarized approach and
other objectives used in the recent literature (\emph{e.g.}\ CRR, ABM, REQ).


There are two main drawbacks to this approach.
First, the preference and scale parameters cannot be set independently, although this derivation reveals the correct decoupling of the temperature into a preference and a scaling of the return estimates.
Second, since $J_S$ only involves an expectation with respect to the expert behavior policy, the policy
cannot evaluate and exploit the $Q$ estimates of actions beyond those taken by the expert.

\subsubsection{Multi-objective RL with DiME}
\label{sec:method_moe}
In this case one separate improved distribution for each objective is obtained and then these distributions are combined via linear weighted :
\begin{align}
    J_{MO}(\theta; s)
    =&\ (1 - \alpha) \int\pi_t(a|s)\exp\left[\frac{Q(a,s)}{\eta_1}\right] \log \pi_{\theta}(a|s)
\notag\\
    &+ \alpha \int\pi_t(a|s)\exp\left[\frac{\log \frac{\pi_{e}(a|s)}{\pi_t(a|s)}}{\eta_2}\right] \log \pi_{\theta}(a|s)
\intertext{Now if we set $\eta_2 = 1$ and rename $\eta \equiv \eta_1$, we obtain:}
    =&\ (1 - \alpha) \int\pi_t(a|s)\exp\left[\frac{Q(a,s)}{\eta}\right] \log \pi_{\theta}(a|s)
    + \alpha \int\pi_{e}(a|s) \log \pi_{\theta}(a|s).
    \label{eq:dime_orl}
\end{align}
Notice the first term yields a gradient that is identical to the usual MPO policy improvement direction, whereas the second term yields one that is identical to behavior cloning.

==> multi_rl_as_inference.tex <==
\section{Multi-Objective Policy Improvement as Inference}
In the main paper, we motivated the multi-objective policy update rules from an intuitive perspective. In this section, we show that our multi-objective policy improvement algorithm can also be derived from the RL-as-inference perspective. In the policy improvement stage, we assume that a $Q$-function for each objective is given, and we would like to improve our policy with respect to these $Q$-functions. The derivation here extends the derivation for the policy improvement algorithm in (single-objective) MPO in \citet{abdolmaleki2018relative} (in appendix) to the multi-objective case.

We assume there are observable binary improvement events, $\{R_k\}_{k=1}^N$, for each objective. $R_k=1$ indicates that our policy has improved for objective $k$, while $R_k=0$ indicates that it has not. Now we ask, if the policy has improved with respect to \emph{all} objectives, i.e., $\{R_k=1\}_{k=1}^N$, what would the parameters $\a$ of that improved policy be? More concretely, this is equivalent to the maximum a posteriori estimate for $\{R_k = 1\}_{k=1}^N$:
\begin{align}
\max_\a p_{\a}(R_1 =1, R_2=1, \dots, R_N=1) \, p(\a) \, ,
\end{align}
where the probability of improvement events depends on $\a$. Assuming independence between improvement events $R_k$ and using log probabilities leads to the following objective:
\begin{align}
\max_\a \sum_{k=1}^N\log p_{\a}(R_k =1) + \log p(\a) \, .
\label{eq:map}
\end{align}
The prior distribution over parameters, $p(\a)$, is fixed during the policy improvement step. We set the prior such that $\pi_\a$ stays close to the target policy during each policy improvement step, to improve stability of learning (\sref{sec:m_step}).
%\begin{align*}
%\max_\theta& \log \prod_{k=1}^N p_{\theta}(R_k =1) + \log p(\theta) \\
%&=\sum_{k=1}^N\log p_{\theta}(R_k =1) + \log p(\theta) \, .
%\end{align*}

%We can compute $p_\a(R_k=1)$ by marginalizing over state and action latent variables:
%\begin{equation}
%    \int_s\mu(s)\int_a p(R_k=1|s,a)\pi_\a(a|s) \diff a \diff s \, ,
%\end{equation}
%After marginalizing out action and state as latent variables of the model and considering random variable dependencies, this is equivalent to optimizing 
%\begin{align*}
%\pi_\textrm{new}&= \argmax_\a  \sum_{k=1}^N\log\Big[ \\&\int_s\mu(s)\int_a p(R_k=1|s,a)\pi_\theta(a|s) \diff a \diff s \Big] +\log p(\theta).
%\end{align*}
%where $\mu(s)$ is the stationary state distribution, which is assumed to be given in each policy improvement step. In practice, $\mu(s)$ is approximated by the distribution of the states in the replay buffer.
%$p(R_k=1|s,a)$ is the likelihood of the improvement event for objective $k$, if our policy chose action $a$ in state $s$. %In other words, $p(R_k=1|s,a)$ defines the probability that in state $s$, taking action $a$ would improve the policy with respect to objective $k$. 
%As we prefer actions with a higher Q-value, this probability density function can be defined as $${p(R_k=1|s,a)} \propto {C(Q_k(s,a))},$$ where $C$ is a monotonically increasing and therefore rank preserving function of the Q-function. This is a sensible choice, as choosing an action with a higher Q-value should have a higher probability of improving the policy in that state.
% Solving for $\theta$ in closed-form is intractable \shnote{add citation}.

We use the standard expectation-maximization (EM) algorithm to efficiently maximize $\sum_{k=1}^N\log p_{\a}(R_k =1)$. The EM algorithm repeatedly constructs a tight lower bound in the E-step, given the previous estimate of $\a$ (which corresponds to the target policy in our case), and then optimizes that lower bound in the M-step. We introduce a variational distribution $q_k(s, a)$ per objective, and use this to decompose the log-evidence $\sum_{k=1}^N\log p_{\a}(R_k =1)$ as follows: % We construct a lower bound on $\sum_{k=1}^N\log p_{\a}(R_k =1)$ by introducing a variational distribution $q_k(s, a)$ per objective using the following standard decomposition,
\begin{align}
\label{eq:decomp}
\sum_{k=1}^N & \log p_{\a}(R_k =1) \\
& = \sum_{k=1}^N \KL(q_k(s,a)\,\|\,p_{\a}(s,a|R_k=1)) \, - \nonumber \\
& \;\;\;\; \sum_{k=1}^N \KL(q_k(s,a)\,\|\,p_{\a}(R_k=1, s, a)) \, . \nonumber
%\mathbb{E}_{q_k(s,a)} \Big[ \log \frac{p_{\a}(R_k=1,s,a)}{q_k(s,a)} \Big] \, .
\end{align}
The second term of this decomposition is expanded as:
\begin{align}
\sum_{k=1}^N & \KL(q_k(s,a)\,\|\,p_{\a}(R_k=1, s, a)) \\
& = \sum_{k=1}^N \mathbb{E}_{q_k(s,a)} \Big[ \log \frac{p_{\a}(R_k=1,s,a)}{q_k(s,a)} \Big] \nonumber \\
& = \sum_{k=1}^N \mathbb{E}_{q_k(s,a)} \Big[ \log \frac{p(R_k=1|s,a)\pi_\a(a|s)\mu(s)}{q_k(s,a)}\Big] \, , \nonumber
\end{align}
%\begin{align}
%\sum_{k=1}^N & \log p_{\a}(R_k =1) = \\
%& \sum_{k=1}^N \KL(q_k(s,a)\,\|\,p_\a(s,a|R_k=1)) \, + \nonumber \\
%& \sum_{k=1}^N\int q_k(s,a)\log \frac{p(R_k=1|s,a)\pi_\a(a|s)\mu(s)}{q_k(s,a)} \diff a \diff s \, . \nonumber
%\end{align}
where $\mu(s)$ is the stationary state distribution, which is assumed to be given in each policy improvement step. In practice, $\mu(s)$ is approximated by the distribution of the states in the replay buffer.
$p(R_k=1|s,a)$ is the likelihood of the improvement event for objective $k$, if our policy chose action $a$ in state $s$.

The first term of the decomposition in Equation \eqref{eq:decomp} is always positive, so the second term is a lower bound on the log-evidence $\sum_{k=1}^N\log p_{\a}(R_k =1)$. $\pi_\a(a|s)$ and $q_k(a|s) = \frac{q_k(s,a)}{\mu(s)}$ are unknown, even though $\mu(s)$ is given. 
In the E-step, we estimate $q_k(a|s)$ for each objective $k$ by minimizing the first term, given $\a = \a'$ (the parameters of the target policy). Then in the M-step, we find a new $\a$ by fitting the parametric policy to the distributions from first step.
%We can now focus on the underlying meaning of $q_k(a|s)$. If in each state we knew which action would lead to a policy improvement, we would fit a policy which outputs that action in each state. However, we do not have access to that knowledge. Instead, in the E-step we  infer a distribution over the actions $q(a|s)$ using the Q-function such that choosing those actions would improve the policy. In the M-step, we then fit a policy to this distribution $q(a|s)$ such that those actions are selected by the newly fitted policy, hence the policy is improved.

\subsection{E-Step}
The E-step corresponds to the first step of policy improvement in the main paper (Sec. 4.2.1). In the E-step, we choose the variational distributions $\{q_k(a|s)\}_{k=1}^N$ such that the lower bound on $\sum_{k=1}^N\log p_{\a}(R_k =1)$ is as tight as possible when $\a=\a'$, the parameters of the target policy. The lower bound is tight when the first term of the decomposition in Equation \eqref{eq:decomp} is zero, so we choose $q_k$ to minimize this term. We can optimize for each variational distribution $q_k$ independently:
\begin{align}
q_k(a|s) &= \argmin_{q} \mathbb{E}_{\mu(s)} \Big[ \KL(q(a|s)\,\|\,p_{\a'}(s,a|R_k=1)) \Big] \nonumber \\
&= \argmin_{q} \mathbb{E}_{\mu(s)} \Big[ \KL(q(a|s)\,\|\,\pi_{\a'}(a|s)) \, -  \nonumber \\
& \qquad\qquad\qquad\quad\;\; \mathbb{E}_{q(a|s)} \log p(R_k=1|s,a)) \Big] \, .
\label{eq:estep}
\end{align}
%this is equivalent to minimizing
%\begin{align} 
%q_k(a|s) & = \argmin_{q} \int \mu(s) \KL(q(a|s)\,\|\,\pi_{\a'}(a|s) )\diff s \nonumber
%- \\& \int \mu(s)\int q(a|s) \log p(R_k=1|s,a))\diff a\diff s \, .
%\label{eq:estep}
%\end{align}

We can solve this optimization problem in closed form, which gives us

$$q_k(a|s) = \frac{\pi_{\a'}(a|s) \, p(R_k=1|s,a)}{\int \pi_{\a'}(a|s) \, p(R_k=1|s,a) \diff a} \, .$$

This solution weighs the actions based on their relative improvement likelihood $p(R_k=1|s,a)$ for each objective. We define the likelihood of an improvement event $R_k$ as $$p(R_k=1|s,a) \propto \exp\Big(\frac{Q_k(s,a)}{\alpha_k}\Big) \, ,$$ where $\alpha_k$ is an objective-dependent temperature parameter that controls how greedy the solution $q_k(a|s)$ is with respect to its associated objective $Q_k(s,a)$. For example, given a batch of state-action pairs, at the extremes, an $\alpha_k$ of zero would give all probability to the state-action pair with the maximum Q-value, while an $\alpha_k$ of positive infinity would give the same probability to all state-action pairs.
In order to automatically optimize for $\alpha_k$, we plug the exponential transformation into \eqref{eq:estep}, which leads to
\begin{align} 
q_k(a|s) & = \argmax_{q} \int \mu(s)\int q(a|s) Q_k(s,a) \diff a \diff s - \nonumber \\
& \qquad \; \alpha_k \int \mu(s) \KL(q(a|s) \,\|\, \pi_{\a'}(a|s) ) \diff s \, .
\end{align}  
If we instead enforce the bound on KL divergence as a hard constraint (which we do in practice), that leads to: 
\begin{align}
\label{eq:findingq}
& q_k(a|s) = \argmax_{q} \int \mu(s)\int q(a|s) Q_k(s,a) \diff a \diff s \\ 
& \qquad \qquad \;\; \textrm{s.t.} \int \mu(s) \KL(q(a|s) \,\|\, \pi_{\a'}(a|s) ) \diff s < \epsilon_k, \nonumber 
\end{align}
where, as described in the main paper, the parameter $\epsilon_k$ defines preferences over objectives. If we now assume that $q_k(a|s)$ is a non-parametric sample-based distribution as in \cite{abdolmaleki2018maximum}, we can solve this constrained optimization problem in closed form for each sampled state $s$, by setting
\begin{equation}
q(a|s) \propto \pi_{\a'}(a|s) \exp\Big(\frac{Q_k(s,a)}{\eta_k}\Big) \, ,
\label{eq:nonparametric}
\end{equation}
where $\eta_k$ is computed by solving the following convex dual function:
\begin{align}
\label{eq:etadual}
&\eta_k=\argmin_{\eta}
\eta\epsilon_k+\\
& \qquad \eta\int\mu(s)\log\int \pi_{\a'}(a|s)\exp\Big(\frac{Q_k(s,a)}{\eta}\Big)\diff a \diff s \, . \nonumber
\end{align}
Equations \eqref{eq:findingq}, \eqref{eq:nonparametric}, and \eqref{eq:etadual} are equivalent to those given for the first step of multi-objective policy improvement in the main paper (Sec. 4.2.1). Please see refer to Appendix D.2 in \cite{abdolmaleki2018maximum} for details on derivation of the dual function.

\subsection{M-Step}
\label{sec:m_step}
After obtaining the variational distributions $q_k(a|s)$ for each objective $k$, we have found a tight lower bound for $\sum_{k=1}^N \log p_\a(R_k=1)$ when $\a=\a'$. We can now obtain the parameters $\a$ of the updated policy $\pi_{\a}(a|s)$ by optimizing this lower bound. After rearranging and dropping the terms in \eqref{eq:map} that do not involve $\a$, we obtain
\begin{align*}
\a^* =& \argmax_{\a} \sum_{k=1}^N\int \mu(s) \int q_k(a|s)\log \pi_\a(a|s)\diff a \diff s \\
   & \qquad \quad + \log p(\a).
\end{align*}
This corresponds to the supervised learning step of policy improvement in the main paper (Sec. 4.2.2).
 
For the prior $p(\a)$ on the parameters $\a$, we enforce that the new policy $\pi_{\a}(a|s)$ is close to the target policy $\pi_{\a'}(a|s)$. We therefore optimize for 
\begin{align*}
&\a^* = \argmax_{\a}  \sum_{k=1}^N \int \mu(s) \int q_k(a|s)\log \pi_\a(a|s) \diff a \diff s \\
& \qquad \textrm{s.t.} \int \mu(s) \KL(\pi_{\a'}(a|s) \,\|\, \pi_{\a}(a|s) ) \diff s < \beta. \nonumber 
\end{align*}
Because of the constraint on the change of the parametric policy, we do not greedily optimize the M-step objective.  See \cite{abdolmaleki2018maximum} for more details.
%Please note that we could also choose the reverse KL in this step. However, our ablation studies show that the forward KL, overall, achieves better performance. Also, the forward KL is compatible with the supervised learning loss that we use for updating the policy.
%Using this approximation, we find a new optimization problem: 
%\begin{align*}
%\a =& \argmax_{\a'} \int \mu(s) \int q(a|s)\log \frac{\pi(a|s,\a') }{q(a|s)}\diff a \diff s  \\ &- \lambda \int \mu(s) \KL(\pi(a|s,\a_t) \,\|\, \pi(a|s,\a')) \diff s
%\end{align*}
%Alternatively we can use a hard constraint to obtain:
%\begin{align*}
%&\a = \argmax_{\a'}  \int \mu(s) \int q(a|s)\log \frac{\pi(a|s,\a')}{q(a|s)} \diff a \diff s \\
%&\textrm{s.t.} \int \mu(s) \KL(\pi(a|s,\a_t) \,\|\, \pi(a|s,\a) ) \diff s < \epsilon \nonumber 
%\end{align*}
%Because of the prior, we do not greedily optimize the M-step objective. 
%Therefore, our approach belongs to the category of generalized expectation maximization algorithms. If we approximate the integrals in the E-step and M-step using the states samples from replay buffer and the action samples from the old policy, we will obtain the update rules we proposed in the paper. %Algorithm \ref{Alg:GradientFree} illustrates this algorithm.

